On the Parameterized Complexity of the Connected Flow and Many Visits TSP Problem

We study a variant of Min Cost Flow in which the flow needs to be connected. Specifically, in the Connected Flow problem one is given a directed graph $G$, along with a set of demand vertices $D \subseteq V(G)$ with demands $\mathsf{dem}: D \rightarrow \mathbb{N}$, and costs and capacities for each edge. The goal is to find a minimum cost flow that satisfies the demands, respects the capacities and induces a (strongly) connected subgraph. This generalizes previously studied problems like the (Many Visits) TSP. We study the parameterized complexity of Connected Flow parameterized by $|D|$, the treewidth $tw$ and by vertex cover size $k$ of $G$ and provide: (i) $\mathsf{NP}$-completeness already for the case $|D|=2$ with only unit demands and capacities and no edge costs, and fixed-parameter tractability if there are no capacities, (ii) a fixed-parameter tractable $\mathcal{O}^{\star}(k^{\mathcal{O}(k)})$ time algorithm for the general case, and a kernel of size polynomial in $k$ for the special case of Many Visits TSP, (iii) a $|V(G)|^{\mathcal{O}(tw)}$ time algorithm and a matching $|V(G)|^{o(tw)}$ time conditional lower bound conditioned on the Exponential Time Hypothesis. To achieve some of our results, we significantly extend an approach by Kowalik et al.~[ESA'20].

==> chapters/demands.tex <==
\section{Parameterized by number of demands}


==> chapters/preliminaries.tex <==
\section{Preliminaries}\label{sec:prel}
The treewidth of a graph is defined as follows. 

\jesper{Define $\Os$, $[b]$, other notation?}
\begin{definition}
	A \emph{tree decomposition} of a graph $G=(V,E)$ is a tree $T$ with nodes $X_1,\dots, X_k$ (where $X_i\subseteq V$ for all $i$) such that
	\begin{itemize}
		\item $X_1\cup\dots\cup X_k=V$;
		\item For all $v\in V$, the nodes containing $v$ form a subtree of $T$;
		\item For every edge $uv$, there is a node containing both $u$ and $v$.
	\end{itemize}
	The width of a tree decomposition is the size of its largest node minus one. The \emph{treewidth} of $G$ is the minimum width of a tree decomposition of $G$.
\end{definition}	 

All graphs in this paper are assumed to be directed. %Throughout the paper, we will work with directed graphs. %In a directed graph $G=(V,E)$, the \textit{multiplicity} of an edge $e\in E$ will be the number of times $e$ appears in the multiset $E$. 
Given a function $f:E\rightarrow \N$, we define $G_f = (V,E')$ to be the graph where $e \in E'$ if and only if $f(e) >0$.

We study the \textsc{Connected Flow} problem, defined as follows.

\defproblem{ \textsc{Connected Flow}}{Digraph $G = (V,E)$, $D \subseteq V$, $\Dem: D\to \N$, $\Dis: E \to \N$, $\Ca: E \to \N\cup\{\infty \}$}{Find a function $f : E \to \N$ such that
	\begin{itemize}		\setlength\itemsep{0em}
		%\item for every $u,v\in V$ such that $(u,v)\not\in E$, $f(u,v)=0$ %\todo{K: added} C: now added it in the definition of f itself :)
		\item $G_f$ is connected, 
		\item for every $v \in V$ we have $\sum_{u \in V} f(u,v)  = \sum_{u \in V} f(v,u)$.
		\item for every $e \in E: f(e) \le \Ca(e)$
		\item for every $v \in D$ we have 
		$\sum_{u \in V} f(u,v) = \Dem(v)$.
	\end{itemize}
	and so as to minimize the value of $\Dis(f) = \sum_{e \in E} \Dis(e)f(e)$}%\label{def:conflow}

Note that $G_f$ in the above definition is Eulerian (since every vertex has the same in and out degree), so it is strongly connected if and only if it is weakly connected.  

We will also work with several problems related to \textsc{Connected Flow}. We define \textsc{Flow} as the \textsc{Connected Flow} problem without the connectivity requirement. \textsc{Flow} can be solved in polynomial time 
\footnote{In Appendix~\ref{app:Definitions} we show that \textsc{Flow} is equivalent to the \textsc{Min Cost Flow} problem, which is polynomial-time solvable.}. 
Note that \textsc{Many Visits TSP} (MVTSP), as defined in \cite{kowalik_et_al:LIPIcs:2020:12932}, is a special case of \textsc{Connected Flow}, where $D=V$ and all capacities are infinite. The formal definitions of these two problems can be found in Appendix~\ref{app:Definitions}.  


\paragraph*{NP-completeness of Connected Flow with few demands.} Even for the case where only two vertices have a specified demand (i.e. $|D| =2$) the \textsc{Connected Flow} problem is NP-complete. This follows from a reduction from the directed vertex-disjoint paths problem, which is known to be NP-complete \cite{karp1975computational}. The details of the reduction can be found Appendix~\ref{app:reductionD}.

\paragraph*{Removing non-demand vertices.}
Given an instance $(G, D, \Dem, \Dis, \Ca)$ of \textsc{Connected Flow} where capacities of all edges are infinite, we can construct an equivalent instance of \textsc{MVTSP}. This is done by removing all vertices in $V\setminus D$ and defining $\Dis'(u,v)$ for $u,v \in D$ as the distance of the shortest $D$-disjoint $(u-v)$ path, if one exists. We keep all demands the same. Since all vertices have a demand,this is indeed an instance of \textsc{MVTSP}. For the complete prove see Appendix~\ref{app:redtoMVTSP}. 

By using the above observation and the $O^*(c^{|D|})$ time algorithm for MVTSP from \cite{kowalik_et_al:LIPIcs:2020:12932}, we obtain the following result.

\begin{corollary} 
	Let $(G, D, \Dem, \Dis, \Ca)$ be an instance of \textsc{Connected Flow} where $cap(e) = \infty$ for all $e \in E(G)$. This instance can be solved in $O^*(c^{|D|})$ time.
\end{corollary}

==> chapters/removedproofs.tex <==
\section{Proofs deferred to appendix}\label{app:proofs}
\begingroup
\def\thenumclaim{\ref{claim:fisflow}}
\begin{numclaim}
	$f$ is a flow for the given instance and $T\subseteq supp(f)$ for all $e \in T$ %, and $\Dis(f)\le \Dis(s)$.
.
\end{numclaim}
\addtocounter{numclaim}{-1}
\endgroup
%\begin{claim} \label{}
%	claim:fisflow
	

%\end{claim}
\begin{proof}
First note that for all $e \in E$: $\min\{r(e),s(e)\} \le f(e) \le  \max\{r(e),s(e)\}$. 
Indeed, if $e \not \in A$, \eqref{eq:f} implies that $r(e) = f(e) = s(e)$. If $e \in A_s$, $r(e)<s(e)$ and we can see from~\eqref{eq:f} that if the multiplicity of $e$ changes, it is because copies of $e$ are added to $r$ to form $f$ (and none are removed). 
Furthermore the multiplicity of $e$ in $A$ is at most $s(e) - r(e)$. Hence $r(e) \le f(e) \le s(e)$. Similarly, if $e \in A_r$, $r(e) > s(e)$ and at most $r(e) - s(e)$ copies of $e$ are removed from $r$ to form $f$. 

Now we prove that for $f$ the flow-preservation constraints and demand constraints are satisfied. Let $C \in C^+$ and let $e,e'$ be two subsequent edges with common vertex $v$ from $C$. If $e \in A_r$ and $e' \in A_s$ (or the other way around), then the in- and out- degrees of the new solution of $v$ do not change, as $e'$ is removed and $e$ is added and they had opposite orientation. Also, if $e, e' \in A_r$, then they are both removed, but since the orientation is the same, both the in and out degree of $v$ go down by one. Note that this can only happen if $v \in D$ by definition of $(s-r)$ directed tours. Therefore, the flow is preserved. In the same way if $e, e' \in A_s$, the flow is preserved. Since for $v \in D$, the total incoming (and total outgoing) edges do not change, the demands are definitely satisfied. Furthermore, the capacity constraints are satisfied since $ f(e) \le  \max\{r(e),s(e)\} \le \Ca(e)$.

Next we show that $T\subseteq supp(f)$. Let $e \in T^+$, then $e \in A_s$ so copies of $e$ are only added to $r$ to form $f$ in~\eqref{eq:f}. Since $e \in T^+$, at least one tour $C \in \mathcal{C}^+$ contains $e$. Hence, $f(e)>0$. 
If $e \in T - T^+$, then $r(e)>0$ and $s(e)>0$. Hence using the fact that $\min\{r(e),s(e)\} \le f(e) $, we conclude that $f(e)>0$. 
%We are left to prove that $\Dis(f)\le \Dis(s)$. For any $C \in \mathcal{C}$ define $\delta(C) = \Dis(A_s \cap C) - \Dis(A_r \cap C)$ as the cost of adding all edges in $A_s \cap C$ and removing all edges in $A_r \cap C$. Notice that $\delta(C)\ge 0 $ for all tours $C \in \mathcal{C}$, as otherwise $r$ would not have been optimal since we could improve it by augmenting along $C$. Hence $\sum_{C \in \mathcal{C}^+} \delta(C) \le \sum_{C \in \mathcal{C}}\delta(C)$ as $\mathcal{C}^+ \subseteq \mathcal{C}$. Therefore:
%$$\Dis(f) = \Dis(r) + \sum_{C \in \mathcal{C}^+} \delta(C) \le  \Dis(r) + \sum_{C \in \mathcal{C}} \delta(C) \le \Dis(s).$$
\end{proof}


\begingroup
\def\thenumclaim{\ref{claim:DP}}
\begin{numclaim}
	Each table entry $T_j(\pi,\mathbf{c}^{\In},\mathbf{c}^{\Out})$ can be computed from all table entries $T_{j-1}$.
\end{numclaim}
\addtocounter{numclaim}{-1}
\endgroup
\begin{proof}
Compute table entries for $j=0$ as follows. Set $T_0(\{\{x_1,\},\dots,\{x_{k'}\}\},\mathbf{0},\mathbf{0}) =1$ and all other entries to $\infty$, as $X'$ is an independent set and so there cannot be any flow as $V_j \setminus X' = \emptyset$. 

Now assume $j> 0$.
For two partitions $\pi, \pi'$ of $X'$, let $\pi'\prec \pi$ denote that for all $S' \in \pi'$ there exists $S\in \pi$ with $S'\subseteq S$.
We compute the values of $T_{j}(\pi,\mathbf{c}^{\In},\mathbf{c}^{\Out})$ as the minimum of the following value over all suitable $h^{\In}_i$, $h^{\Out}_i$ and $\pi'$:
\[T_{j-1}(\pi',\mathbf{c}^{\In}-\mathbf{h}^{\In},\mathbf{c}^{\Out}-\mathbf{h}^{\Out}) + \sum_{i=1}^{k'} \left( h^{\In}_i \cdot \Dis(b_{j-1},x_i) + h^{\Out}_i\cdot \Dis(x_i,b_{j-1})\right).
\]
Here we interpret $h^{\In}_i$ as the multiplicity of the edge $(b_j,x_i)$ and $h^{\Out}_i$ as the multiplicity of the edge $(x_i,b_j)$. Hence, we require that  $\pi'\prec \pi$ and if there exist $S_1, \dots S_l \in \pi'$ s.t. $S_1\cup \dots \cup S_l \in \pi$, then $S_1,\dots,S_l$ are connected to each other in $\pi$ through $b_j$. Furthermore, we require that the solution is flow preserving in $b_j$, i.e. $\sum_{i =1}^{k'} h^{\In}_i = \sum_{i =1}^{k'} h^{\Out}_i$ and $\sum_{i =1}^{k'} h^{\In}_i = \Dem(b_j)$ if $b_j \in D$. Lastly, the capacity constraints must hold, which means that $h^{\In}_i \le \Ca(b_j,x_i)$ and $h^{\Out}_i \le \Ca(x_i,b_j)$.

Notice that with this recurrence, the table entries are computed correctly as only the vertex $b_j$ was added, compared to the table entries $T_{j-1}$. Therefore we may assume that only the edges incident to $b_j$ were added to another solution for some table entry in $T_{j-1}$. 
\end{proof}

\begingroup
\def\thenumclaim{\ref{claim:kernel}}
\begin{numclaim}
There exists an optimal solution $f'$ of the \textsc{MVTSP} instance such that for all $i,j \in [k]$, $b \in R_{ij}$ and $x_l \in X$ it holds that $r(x_l,b) = f'(x_l,b)$ and $r(b,x_l) = f'(b,x_l)$.
\end{numclaim}
\addtocounter{numclaim}{-1}
\endgroup

\begin{proof}
We build this $f'$ iteratively from $f$, by removing any edge between $b \in R_{ij}$ and $x_l$ that shouldn't exist.

Throughout we will retain optimality and connectivity for $f'$. Furthermore, after each step, the solutions $r$ and $f'$ differ at at most $8k^2$ edges. 

Let us consider $b \in R_{ij}$ and suppose that $f'(x_l,b) >0$ for some $l \not = i$. Note that we can tackle the case where $f'(b,x_l)>0$ for some $l\in [k]\setminus \{j\}$ with the same steps as that follow. As at most $8k^2$ edges are different between $r$ and $f'$, there are vertices $v,w \in \overr{A_{ij}}(l)$ such that all  of the edges adjacent to $v$ and $w$ have the same multiplicities in $r$ and $f'$, i.e. $f'(u,v) = r(u,v)$. Note that indeed $|\overr{A_{ij}}(l)| = 8k^2 +2$ as $R_{ij} \not = \emptyset$. 

Define flow $f''$ with at most the same costs as $f'$ by removing one copy of the edges $(x_l,b)$ and $(x_i,v)$ and adding one copy of the edges $(x_i,b)$ and $(x_l,v)$, see Figure~\ref{fig:kernel}. As $b \not \in \overr{A_{ij}}(l)$ and $v \in \overr{A_{ij}}(l)$, the cost of $f''$ is indeed at most the cost of $f'$. We now argue that $f''$ is connected. 

As $f'$ is a solution, it must be connected. Removing $(x_l,b)$ and $(x_i,v)$ from $f'$ can create something unconnected, but proving that the pairs $x_l,b$ and $x_i,v$ are connected in $f''$ proves $f''$ to be connected as well. As $(x_i,b)$ and $(x_l,v)$ are added, it is sufficient to prove $v$ and $x_i$ to be connected in $f''$. This is true as there exists edges $(x_i,w)$, $(w,x_j)$ and $(v,x_j)$, so $f''$ must be connected. Finally, notice that the number of edges that differ between $f''$ and $r$ has not changed. Hence, continue with setting $f' = f''$ and repeat until $f'$ has the required properties.
\begin{figure}[ht!]
\centering
\begin{minipage}{.45\textwidth}
\centering
\scalebox{1}{\input{img/Kernel1}}
\end{minipage} \hspace{20pt}
\begin{minipage}{.45\textwidth}
\centering
\scalebox{1}{\input{img/Kernel2}}
\end{minipage}
\caption{Adjusting flow $f'$, depicted on the left, to get flow $f''$, depicted on the right. The blue edges are replaced by the red edges, the rest of the solutions are equal. The vertex $w$ assures the new solution remains connected} 
\label{fig:kernel}
\end{figure}
\end{proof}





==> chapters/treewidthsummary.tex <==
\section{Treewidth} \label{sec:TreeSum}

When parameterized by treewidth, we get a tight classification of the problem by heavily using (fairly standard) methodology from previous papers. In particular,  we have a dynamic programming algorithm which establishes the following result:

\begin{theorem}\label{thm:TwDP}
Let $M$ be an upper bound on the demands in the input graph $G$, and suppose a tree decomposition of width $\tw$ of $G$ is given. Then a \textsc{Connected Flow} instance with $G$ can be solved in time $|V(G)|^{\Oh(\tw)}$ and an \textsc{MVTSP} instance with $G$ can be solved in time $\min\{|V(G)|,M\}^{\Oh(\tw)}|V(G)|^{\Oh(1)}$.
\end{theorem}

The algorithm builds a table with entries describing partial solutions. These entries are indexed by the in and out degrees of vertices of bags in a tree decomposition, as well as a partition of the bag which describes the connectivity. It turns out that this running time is essentially optimal:

\begin{theorem}\label{thm:3SatRed}
Let $M$ be an upper bound on the demands in a graph $G$. Then \textsc{MVTSP} cannot be solved in time $f(\pw)\min\{|V(G)|,M\}^{o(\pw)}|V(G)|^{\Oh(1)}$, unless ETH fails.
\end{theorem}

Note that this theorem implies Theorem~\ref{thm:tw=hard}. We prove this upper bound using a reduction from \textsc{3-CNF-SAT}. The main idea is to encode assignments of sets of variables as flow through a path, where the amount of flow encodes a partial assignment of a group of variables. We then build so-called scanner gadgets which detect whether a clause is satisfied. This reduction is based on ideas from Cygan et al.~\cite{DBLP:journals/corr/abs-1211-1506}.
Details are deferred to Appendix~\ref{sec:pathw}.
